Can Virtual Reality Protect Users from Keystroke Inference Attacks?

Virtual Reality (VR) has gained popularity by providing immersive and interactive experiences without geographical limitations. It also provides a sense of personal privacy through physical separation. In this paper, we show that despite assumptions of enhanced privacy, VR is unable to shield its users from side-channel attacks that steal private information. Ironically, this vulnerability arises from VR's greatest strength, its immersive and interactive nature. We demonstrate this by designing and implementing a new set of keystroke inference attacks in shared virtual environments, where an attacker (VR user) can recover the content typed by another VR user by observing their avatar. While the avatar displays noisy telemetry of the user's hand motion, an intelligent attacker can use that data to recognize typed keys and reconstruct typed content, without knowing the keyboard layout or gathering labeled data. We evaluate the proposed attacks using IRB-approved user studies across multiple VR scenarios. For 13 out of 15 tested users, our attacks accurately recognize 86%-98% of typed keys, and the recovered content retains up to 98% of the meaning of the original typed content. We also discuss potential defenses.

==> Makefile <==
LATEX=pdflatex

BIBTEX=bibtex
BIBFILE=ref.bib
PAPER=keystroke

TEXFILES = 	keystroke.tex \
	tex/intro.tex \
	tex/background.tex \
	tex/threat.tex\
	tex/alternatives.tex \
	tex/overview.tex \
	tex/study.tex \
	tex/noise.tex \
	tex/attack.tex \
	tex/defense.tex \
	tex/conclusion.tex \
	tex/appendix.tex 

FIGS = $(wildcard fig/*.pdf)
TABLES = $(wildcard table/*.tex)

all:   $(PAPER).pdf
	open $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) $(PAPER)

$(PAPER).pdf: $(TEXFILES) $(BIBFILE) $(FIGS) $(TABLES)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

compress: $(TEXFILES) $(BIBFILE) $(FIGS) $(TABLES)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)
	$(LATEX)  $(PAPER)
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE -dQUIET -dBATCH -sOutputFile=$(PAPER)-compressed.pdf $(PAPER).pdf

embedfonts: $(TEXFILES) $(BIBFILE) $(FIGS) $(TABLES)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)
	$(LATEX)  $(PAPER)
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dEmbedAllFonts=true -sOutputFile=$(PAPER)-embedfonts.pdf $(PAPER).pdf

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out *.fdb_latexmk *.fls *.synctex.gz

